Multidimensional Bayesian IRT Model for Hierarchical Latent Structures

It is reasonable to consider, in many cases, that individuals' latent traits have a hierarchical structure such that more general traits are a suitable composition of more specific ones. Existing item response models that account for such hierarchical structure feature have considerable limitations in terms of modelling and/or inference. Motivated by those limitations and the importance of the theme, this paper aims at proposing an improved methodology in terms of both modelling and inference to deal with hierarchically structured latent traits in an item response theory context. From a modelling perspective, the proposed methodology allows for genuinely multidimensional items and all of the latent traits in the assumed hierarchical structure are on the same scale. Items are allowed to be dichotomous or of graded response. An efficient MCMC algorithm is carefully devised to sample from the joint posterior distribution of all the unknown quantities of the proposed model. In particular, all the latent trait parameters are jointly sampled from their full conditional distribution in a Gibbs sampling algorithm. The proposed methodology is applied to simulated data and a real dataset concerning the Enem exam in Brazil.

==> caption/CHANGELOG <==
Changes made in the caption package bundle
==========================================

Please note that this document does not reflect bugfix-releases, and that the dates given are the dates of the release w/o bugfixes.

If you are interested in a complete changelog -- including bugfixes -- process the dtx files with \RecordChanges and \PrintChanges.


caption package
---------------

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added

v3.4 (2019/09/11)
- Label format `autodot' added (for usage within documents using KOMA-Script document class)
- Label format `unnumbered' added
- \ContinuedFloat renamed to \continuedfloat (since this is not a preamble command)
- \caption will always be re-defined now, unless `compatibility' is set to `v1' (or an incompatible package is loaded)


bicaption package
-----------------

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added

v1.2 (2016/03/27)
- \DeclareLangDependantCaptionOption added


ltcaption package
-----------------

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
------------------

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption

v1.2 (2018/05/13)
- Values `B' and `T' for the optional argument <outer-pos> added to the environments `subfigure' and `subtable'

v1.3 (2019/08/31)
- New command \subfloat for easy transition from the `subfig' package


totalcount package
------------------

v1.0 (2008/03/09)
- 1st published version



==> caption/README <==
==========================================================================

The `caption' package bundle
Release 2020-07-20
Copyright (C) 1994-2020 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  https://gitlab.com/axelsommerfeldt/caption

If you need help for installation please visit:
  https://texfaq.org/FAQ-inst-miktexstar
  https://texfaq.org/FAQ-installthings
  https://texfaq.org/FAQ-privinst

If you need help using these packages please visit:
  https://latex.org/forum/
  https://tex.stackexchange.com/
  https://golatex.de/               (German)
  https://texwelt.de/               (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  https://gitlab.com/axelsommerfeldt/caption/issues (preferred)
or send an e-mail to
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.4 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.2 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.3 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

Note: The `newfloat' package was removed from this package bundle and was
uploaded to CTAN as stand-alone package.

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)

